Approximate resilience, monotonicity, and the complexity of agnostic learning

A function $f$ is $d$-resilient if all its Fourier coefficients of degree at most $d$ are zero, i.e., $f$ is uncorrelated with all low-degree parities. We study the notion of $\mathit{approximate}$ $\mathit{resilience}$ of Boolean functions, where we say that $f$ is $\alpha$-approximately $d$-resilient if $f$ is $\alpha$-close to a $[-1,1]$-valued $d$-resilient function in $\ell_1$ distance. We show that approximate resilience essentially characterizes the complexity of agnostic learning of a concept class $C$ over the uniform distribution. Roughly speaking, if all functions in a class $C$ are far from being $d$-resilient then $C$ can be learned agnostically in time $n^{O(d)}$ and conversely, if $C$ contains a function close to being $d$-resilient then agnostic learning of $C$ in the statistical query (SQ) framework of Kearns has complexity of at least $n^{\Omega(d)}$. This characterization is based on the duality between $\ell_1$ approximation by degree-$d$ polynomials and approximate $d$-resilience that we establish. In particular, it implies that $\ell_1$ approximation by low-degree polynomials, known to be sufficient for agnostic learning over product distributions, is in fact necessary. Focusing on monotone Boolean functions, we exhibit the existence of near-optimal $\alpha$-approximately $\widetilde{\Omega}(\alpha\sqrt{n})$-resilient monotone functions for all $\alpha>0$. Prior to our work, it was conceivable even that every monotone function is $\Omega(1)$-far from any $1$-resilient function. Furthermore, we construct simple, explicit monotone functions based on ${\sf Tribes}$ and ${\sf CycleRun}$ that are close to highly resilient functions. Our constructions are based on a fairly general resilience analysis and amplification. These structural results, together with the characterization, imply nearly optimal lower bounds for agnostic learning of monotone juntas.

==> amplify.tex <==
% !TEX root =main2.tex
\section{Proof of Theorem \ref{thm:amplification-lemma}}
\label{sec:amplification-lemma}
We write $\dist(f,g)$ to denote $\Pr_{\bx}[f(\bx)\ne g(\bx)]$.
\begin{lemma}
Given $F,G : \bits^m\to\bits$, and balanced $f,g : \bits^n\to\bits$, we have
\[ \dist(F\circ f, G \circ g) \le \dist(F,G) + \NS_\delta[F], \]
where $\delta = \dist(f,g)$.
\end{lemma}

\begin{proof}
We first apply the the triangle inequality and note that
\[ \dist(F\circ f, G\circ g) \le \dist(F\circ f,  F\circ g) + \dist(F\circ g, G\circ g). \]
Since $g$ is balanced, we have that $g(\bx^1),\ldots,g(\bx^m)$ is uniformly distributed on $\bits^m$ when $\bx^1,\ldots,\bx^m$ are uniformly distributed on $\bits^n$ , and therefore the second distance is exactly $ \dist(F,G)$.  For the second distance, we note that $f(\bx)$ and $g(\bx)$ are uniformly random bits satisfying $\Pr_{\bx}[f(\bx)\ne g(\bx)] = \delta$, and so
\[ \dist(F\circ f, F\circ g) = \Prx_{\y,\z}[F(\y) \ne F(\z)], \]
where $\y$ is uniform in $\bits^m$ and $\z$ is obtained from $\y$ by independently flipping each of its coordinates with probability $\delta$.  Since the probability on the right hand side is precisely $\NS_\delta[F]$,  this completes the proof.
\end{proof}

Using the union bound, we have

\[
\NS_{\delta}[F] \leq \delta \sum_{i=1}^n \Prx_{\bx}[F(\bx) \neq F(\bx^{\oplus i})] = \delta \cdot \Inf[F] = \dist(f,g) \cdot \Inf[F]
\]

where $\bx^{\oplus i}$ is the string $\bx$ with the $i$-th bit flipped, and $\delta = \dist(f,g)$ as in the previous lemma.  This, along with a straightforward recursion, yields the following corollary.

\begin{corollary}
\label{cor:distance-amplification}
Given $F,G : \bits^m\to\bits$, and balanced $f,g : \bits^n\to\bits$, we have
\[ \dist(F\circ f, G \circ g) \le \dist(F,G) + \dist(f,g)\cdot \Inf[F]. \]
Consequently, if we let $f_0 = f$ and $g_0 = g$ and consider the recursively-defined functions $f_k = F\circ f_{k-1}$ and $g_k = G\circ g_{k-1}$ for all $k\in \N$, we have:
\[ \dist(f_k, g_k) \le (\dist(F,G) + \dist(f,g))\cdot \Inf[F]^k.\]
\end{corollary}

\begin{lemma}
\label{lem:resilience-amplification}
If $G$ is $d_1$-resilient and $g$ is $d_2$-resilient, then $G\circ g$ is $(d_1d_2)$-resilient.
\end{lemma}

\begin{proof}
By linearity of the Fourier transform it suffices to prove this claim when $G = {\sf PAR}_{d_1}$, the parity of $d_1$ many variables.  Every Fourier coefficient in the spectral support of ${\sf PAR}_{d_1} \circ g$ is of the form
\[ \prod_{i\in [d_1]} \widehat{g}(S_i) \chi_{S_i}(x^i), \quad S_i \in \mathrm{supp}(\widehat{g}), \]
and so the claim follows.
\end{proof}

Combining Corollary \ref{cor:distance-amplification} and Lemma \ref{lem:resilience-amplification} yields Theorem \ref{thm:amplification-lemma}.

%we have shown:
%\begin{proposition}
%\label{prop:amplification-lemma}
%Let $F,G:\bits^m\to\bits$.  Let $f_0,g_0:\bits^n\to\bits$ be balanced Boolean functions, and suppose $G$ is $d_1$-resilient and $g$ is $d_2$-resilient.  Consider the recursively-defined functions $f_k = F\circ f_{k-1}$ and $g_k = G\circ g_{k-1}$ for all $k \in \N$.  Then:
%\begin{enumerate}
%\item $f_k$ and $g_k$ are functions over $m^k \cdot n$ variables,
%\item $g_k$ is $( (d_1+1)^k\cdot (d_2+1)-1)$-resilient,
%\item $\dist(f_k, g_k) \le (\dist(F,G) + \dist(f,g))\cdot \Inf[F]^k.$
%\end{enumerate}
%\end{proposition}

%\Pr[ T\circ g^{\otimes m}\neq H \circ g^{\otimes m} ].$$
%Since $g$ is balanced, $g(x^1)\circ \cdots \circ g(x^m)$ is uniformly distributed in $\bits^m$, and the second probability is exactly $\Pr[ T\neq H] \leq \delta_1$.  For the first probability, note that
%\begin{align*}
%\Pr[ T\circ f^{\otimes m} \neq T \circ g^{\otimes m} ] & \leq
%\Pr_{x\sim y}[ T(x) \neq T(y) ]\\
%& \leq
%2\delta_2 \cdot \Inf[T],
%\end{align*}
%where $x$ is uniform in $\bits^m$ and each $y_i$ is independently set to $x_i$ with probability $1-\delta_2$  and $-x_i$ with probability $\delta_2$. The second inequality follows from Fact~?.
%\end{proof}
%We now apply Lemma \ref{lem:compose} repeatedly.  Define functions $f_i,g_i$ recursively:
%$$f_i  = T\circ f_{i-1}^{\otimes m}$$
%$$g_i = H\circ g_{i-1}^{\otimes m}$$
%If $f_{i-1},g_{i-1}$  are both over $n_{i-1}$ variables, then $f_i,g_i$ are over $n_i = m\cdot n_{i-1}$ variables, and
%an application of Lemma \ref{lem:compose} gives
%$$\Pr[ f_i \neq g_i ] \leq \delta_1 + \delta_2^{(i-1)} \Inf[T],$$
%where $\delta_2^{(i-1)} = \Pr[ f_{i-1} \neq g_{i-1} ]$.  Expanding gives that
%\begin{align*}
%\delta^{(i)}_2  &= \delta_1 \cdot \sum_{j=0}^{i-1} \Inf[T]^j + \delta^{(0)} \Inf[T]^i \\
%& \leq \Inf[T]^i (i \cdot \delta_1+\delta_2^{(0)}),
%\end{align*}
%where the inequality holds because $\Inf[T] \geq 1.$

%Consider balanced $T,H$ and $f_0,g_0$ that satisfy:
%\begin{itemize}
%\item $\sum_{|S|\leq d(m)} \widehat{H}(S)^2 =0$
%\item $\delta_1 \equiv \Pr[T\neq H] = O(\log m/\sqrt{m})$
%\item $\Inf[T] \leq C\log m$
%\item $\delta_2^{(0)} \equiv \Pr[f_0\neq g_0]=O(\log n_0/\sqrt{n_0})$ and
%\item $\sum_{|S|\leq d(n_0)} \widehat{g}_0(S)^2=0$
%\end{itemize}
%Then, we obtain $g_i$ and $f_i$ over $m^i\cdot n_0$ variables, where $g_i$ is $d(m)^i \cdot d(n_0)$-resilient, and:
%$$\Pr[ f_i\neq g_i ] \leq  (C\log m)^i (i\frac{ \log m}{\sqrt{m}} + \frac{\log n_0}{\sqrt{n_0}}).$$
%If we set $m=n_0=n$ and
%$i=c \log n/\log \log n$, we obtain $g_i$ such that:
%\begin{enumerate}
%\item $\sum_{|S|\leq d'} \widehat{g_0}(S)^2 =0$ where $d'=d(n)^{c \log n/\log \log n} = n^{\Omega(1)}$ (if we take $d(n)=O(\log n/\log \log n)$),
%\item $\Pr[f_i\neq g_i ] \leq O(n^{c'-1/2}).$
%for some $c'<c$.
%\end{enumerate}
%The number of variables is $n_i=m^{i+1} = 2^{c\log^2 n/\log \log n}$, while the resilience is
%at least $2^{\Omega(\sqrt{\log n_i})}$.

